An Invariant Learning Characterization of Controlled Text Generation

Controlled generation refers to the problem of creating text that contains stylistic or semantic attributes of interest. Many approaches reduce this problem to training a predictor of the desired attribute. For example, researchers hoping to deploy a large language model to produce non-toxic content may use a toxicity classifier to filter generated text. In practice, the generated text to classify, which is determined by user prompts, may come from a wide range of distributions. In this paper, we show that the performance of controlled generation may be poor if the distributions of text in response to user prompts differ from the distribution the predictor was trained on. To address this problem, we cast controlled generation under distribution shift as an invariant learning problem: the most effective predictor should be invariant across multiple text environments. We then discuss a natural solution that arises from this characterization and propose heuristics for selecting natural environments. We study this characterization and the proposed method empirically using both synthetic and real data. Experiments demonstrate both the challenge of distribution shift in controlled generation and the potential of invariance methods in this setting.

==> preamble/draft.tex <==
\section{An invariant learning perspective of controlled generation}
In this section, we will use the language of causality to characterize various distribution shift problems in controlled generation.
We will provide a definition of control and diversity.
We will see that an increase in control might come at a cost of diversity.
We will also see that if we enforce invariance, we can increase the control, without the cost of diversity.

\subsection{Problem Formulation.}
\paragraph{Setup. }We assume that we observe $p(x)$ which is a pre-trained language model.
The target attribute is denoted by $y$, e.g., toxicity.
We also observe $(x_i, y_i, e_i) \sim q(x_i, y_i, e_i)$.

For simplicity, we will approximate \cref{eq:estimand} via rejection sampling, though the general issue of distribution shift applies regardless of methods used for the approximation.
In more details, we fit 
We have a predictor $\hat{f}$ that maps from the text $x$ to the toxicity $y$.
We do controlled generation through rejection sampling using this predictor.
In the binary case, we might use the predictor to approximate the controlled distribution,
\begin{align}
p(x \g y=0) \approx p(x \g  \hat{f}(x) < 0.5).
\end{align}
% For notation convenience, we will use $\hat{g}(x)$ to denote $p(x \g  \hat{f}(x) < 0.5)$.



% is the following really necessary?
% \paragraph{A causal formulation}
% We will a take causal view of this generating process.
% % As shown in \cref{fig:causal_graph}, $x$ denotes text.
% % The variable $y$ denotes toxicity.
% % The latent variables $\mathbf{z}$ are some causal factors of the text $x$.
% % For intuition, we can think of them as ``topics", ``sentiments", or ``content".
% Using the language of a structural causal model (SCM) \cite{pearl2000causality}, the underlying data generating process is
% \begin{align}
% z_y := f_{z_y}(u_{z_y}); \hspace{2em} z_{\Bar{y}} := f_{z_{\Bar{y}}}(u_{z_{\Bar{y}}});\hspace{2em} 
% x := f_x(z_y, z_{\Bar{y}}, u_x), \hspace{2em} y := f_y(x, u_y),    \label{eq:scm}
% \end{align}
% where $u_{z_y}$, $u_{z_{\Bar{y}}}$, $u_x$, $u_y$ are independent exogenous variable, and the functions $f$ are deterministic functions.

% \paragraph{Control.} To assess control, we might ask, in the controlled distribution, what is the probability of seeing a toxic sample.
% \begin{align}
% \EE{p(x, y)}{\mathbb{y=0} \g \hat{f}(x) =0 },
% \end{align}

% where $m(y)$ is some measurement of the outcome variable.

% The diversity of the controlled generation is much difficult to measure. \citet{yang2021fudge} use the number of unique unigrams, bigrams, and trigrams across all samples. add more cites.




% Here we consider a new measurements of diversity, which is capture by these latent factors $\mathbf{z}$. 
% In this conditional model, we say that the controlled distribution is preserves its conditional distribution of the latent codes if
% \begin{align}
% p(z\g y=0) = g(z). \label{eq:diversity}
% \end{align}

% Often time there are statistical or causal relationships between the factors.
% For example, sentiment and topics could be confounded by the social environments.


%\subsection{failure modes}
% defintion of control
\paragraph{Definition of control. }To assess control, we might ask, in the controlled distribution, what is the probability of seeing a toxic sample.
\begin{align}
\EE{p(x, y)}{m(y)} = \int \int \underbrace{\mathbb{1}(y=0)}_{term 1} \underbrace{p(y \g x)}_{term 2} \underbrace{p(x\g \hat{f}(x) < 0.5)}_{term 3}dydx. \label{eq:control_loss}
\end{align}

\paragraph{Why Control is hard}
The goal is to learn a predictor $\hat{f}$, such that it can optimize for control.
Term 1 is the loss for data pair $(x, y)$.
Term 2 is the probability is toxic given the text.
Term 3 is the distribution of the text.
As we can see here, if the function $\hat{f}$ restrict to the probability space that the predictor has high confidence of being non-toxic, then it will reduce the probability of the model produce toxic sample.

% why is optimizing for control is hard.
%\input{template/graphs/discriminator}

However, an increase in the control may come at a trade off of diversity.
There are many different measurements of diversity.
For example, they can be causes of the text, such as topics, or sentiment.
Or some measurement of the text, such as style.


\paragraph{Control diversity trade off. }
We further de-compose the loss into the following,
\begin{align}
\EE{p(x, y)}{m(y) \g \hat{f}(x) <0.5} = \int_x \int_z \underbrace{\E{\mathbb{1}(y=0)\g x, z}}_{term 1} \underbrace{p(z , x\g \hat{f}(x) <0.5)}_{term 2}dzdx. \label{eq:control_loss}
\end{align}

If $z \indep y \g x$, then term 1 is not dependent on $z$.Therefore, any improvement on the predictor is independent of the latent variable $z$. In other words, we should encode the inductive biases that 


\begin{assumption}{causal sufficiency}\label{as:sufficiency}

there exist a representation $\phi(x)$, such that 
\begin{align}
p(y \g \phi(x), e) = p(y \g \phi(x)) \forall e    
\end{align}
\end{assumption}


\begin{assumption}{overlap}\label{as:overlap}
there's overlap between $p(x) $ and $q(x)$
\end{assumption}

If \cref{as:sufficiency} and \cref{as:overlap} both hold, an invariant predictor can optimize for control without the cost of diversity.


% method that actually 
Finding an invariant representation is equivalent as finding an invariant predictor.
If we have invariant predictor, then we can propagate errors from the predictor to the resulting probability distribution.
To address this problem, we can train an invariant predictor through
More concretely, assume that we have multiple datasets $D_e := \{(x_i^e, y_i^e)\}^{n_e}_{i=1}$.
To train an invariant predictor,
  \begin{align}
    \label{eq:invariance}
    f \in \argmin_{f: \mathcal{X} \rightarrow \mathcal{Y}} R^{e}(f_{\theta}(x), y) \quad \textrm{for all \,} e \in \mathcal{E},
  \end{align}\setlength{\textfloatsep}{0pt}
  
 
To optimize for \cref{eq:invariance}, one way of doing it is through rex \citep{krueger2021out}
\begin{align}
R_{v-rex}(f) = \beta* Var({R_1(f), ... R_m(f)}) + \sum^m_{e=1} R_e(f)\label{eq:rex}
\end{align}
  
% \subsection{Diversity as a byproduct of invariance}
% % \subsection{spurious correlations in the generator}
% this part needs work.

% If we have an invariant predictor, using it, we can achieve control.
% However, we might be interested in the diversity.
% Instead of conditional on only the non-toxic text, we might want the diversity of the text to be akin to the unconditional distribution.


% It is impossible to do without further assumptions on how the factors relate to each other.
% OTOH, it is impossible to specify an accurate causal graph about various causal factors when the domain is all of the internet.


% \begin{align}
% p(x \g do(z_y) ) &= \int p(x \g z_y, z_{\Bar{y}}) p(  z_{\Bar{y}})dz\\
% &= int p(x \g z_y, z_{\Bar{y}}) \frac{p(z_{\Bar{y}} )}{p(z_{\Bar{y}} \g y=0)}p(z_{\Bar{y}} \g y=0)dz
% \end{align}


% We might also be able to do some

% \begin{align}
% p(x \g do(z_y) ) &= p(x \g do(z_y) )
% &= int p(x \g z_y, z_{\Bar{y}}) \frac{p(z_{\Bar{y}} )}{p(z_{\Bar{y}} \g y=0)}p(z_{\Bar{y}} \g y=0)dz
% \end{align}
% construct $\Tilde{p}(x)$.

% However, as humans are the data generator of the text, we can easily ``intervene" or change the text by doing some type of data augmentation. 

% Formally, if we inject some noise to the factor, or by directly intervening on the factor, we can yield these causal factors to be independent.
% \begin{align}
% do(z_y := \Tilde{f}_{z_y}(u_{a}, u_{z_y})    )
% \end{align}
% where $u_a$ is some new exogenous noise.



==> preamble/format.tex <==
% ===== fonts

\usepackage[T1]{fontenc}
\usepackage[full]{textcomp}
\usepackage{newtxtext}
%\usepackage{ccfonts}
% \usepackage{amssymb}
% \usepackage[bb=mt,cal=mt]{mathalpha}

% ====== math

\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{thmtools}
\usepackage{mathtools}

% ===== spacing and text

\usepackage[parfill]{parskip}
\setlength{\parindent}{0pt}
\setlength{\parskip}{2ex plus 0.2ex minus 0.2ex}
\usepackage{afterpage}
\usepackage{setspace} % e.g. \onehalfspacing

% ===== sections and title

\RequirePackage[bf,tiny]{titlesec}

% ===== geometry

\usepackage[
paper  = letterpaper,
left   = 1.0in,
right  = 1.0in,
top    = 1.0in,
bottom = 1.0in,
]{geometry}


%%% Local Variables:
%%% mode: plain-tex
%%% TeX-master: t
%%% End:


==> preamble/math.tex <==

% # PROBABILITY	

\newcommand{\g}{\,\vert\,}	
\newcommand{\s}{\,;\,}	
\newcommand{\indpt}{\protect\mathpalette{\protect\independenT}{\perp}}	
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}	
\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}	
\newcommand{\EE}[2]{\mathbb{E}_{#1}\left[#2\right]}	
\newcommand{\var}[1]{\textrm{Var}\left[#1\right]}	
\newcommand{\h}[1]{\mathbb{H}\left( #1 \right)}	
\newcommand{\kl}[1]{\mathrm{KL}\left(#1\right)}	

% # DISTRIBUTIONS	

\newcommand{\mult}{\mathrm{Mult}}	
\newcommand{\dir}{\mathrm{Dir}}	
\newcommand{\discrete}{\mathrm{Discrete}}	
\newcommand{\Bern}{\mathrm{Bernoulli}}	
\newcommand{\DP}{\mathrm{DP}}	
\newcommand{\GP}{\mathrm{GP}}	
\newcommand{\Bet}{\mathrm{Beta}}	
\newcommand{\pois}{\mathrm{Pois}}	

% # CALLIGRAPHY	

\newcommand{\cL}{\mathcal{L}}	
\newcommand{\cN}{\mathcal{N}}	
\newcommand{\cD}{\mathcal{D}}	
\newcommand{\cE}{\mathcal{E}}	

% # USEFUL	

\newcommand{\RR}{\mathbb{R}}	
\newcommand{\half}{\frac{1}{2}}	
\newcommand{\new}{\mathrm{new}}	
\newcommand{\const}{\mathrm{const.}}	
\newcommand{\dd}{\mathrm{d}}	
\newcommand{\ddx}[1]{\frac{\partial}{\partial #1}}	
\newcommand{\dfdx}[2]{\textstyle \frac{\partial #1}{\partial #2}}	
\newcommand\dif{\mathop{}\!\mathrm{d}}	
\newcommand{\ind}{\mathbb{1}}	
\newcommand{\rmp}{\mathrm{p}}	
\newcommand{\prob}{\mathrm{P}}	

\newcommand{\epehe}{\mathbf{\epsilon_{\text{PEHE}}}}	

\newcommand{\eate}{\mathbf{\epsilon_{\text{ate}}}}	
% # BOLD MATHEMATICS	

\DeclareRobustCommand{\mb}[1]{\ensuremath{\boldsymbol{\mathbf{#1}}}}	

\newcommand{\mba}{\mathbf{a}}	
\newcommand{\mbb}{\mathbf{b}}	
\newcommand{\mbc}{\mathbf{c}}	
\newcommand{\mbd}{\mathbf{d}}	
\newcommand{\mbe}{\mathbf{e}}	
%\newcommand{\mbf}{\mathbf{f}}	
\newcommand{\mbg}{\mathbf{g}}	
\newcommand{\mbh}{\mathbf{h}}	
\newcommand{\mbi}{\mathbf{i}}	
\newcommand{\mbj}{\mathbf{j}}	
\newcommand{\mbk}{\mathbf{k}}	
\newcommand{\mbl}{\mathbf{l}}	
\newcommand{\mbm}{\mathbf{m}}	
\newcommand{\mbn}{\mathbf{n}}	
\newcommand{\mbo}{\mathbf{o}}	
\newcommand{\mbp}{\mathbf{p}}	
\newcommand{\mbq}{\mathbf{q}}	
\newcommand{\mbr}{\mathbf{r}}	
\newcommand{\mbs}{\mathbf{s}}	
\newcommand{\mbt}{\mathbf{t}}	
\newcommand{\mbu}{\mathbf{u}}	
\newcommand{\mbv}{\mathbf{v}}	
\newcommand{\mbw}{\mathbf{w}}	
\newcommand{\mbx}{\mathbf{x}}	
\newcommand{\mby}{\mathbf{y}}	
\newcommand{\mbz}{\mathbf{z}}	

\newcommand{\mbA}{\mathbf{A}}	
\newcommand{\mbB}{\mathbf{B}}	
\newcommand{\mbC}{\mathbf{C}}	
\newcommand{\mbD}{\mathbf{D}}	
\newcommand{\mbE}{\mathbf{E}}	
\newcommand{\mbF}{\mathbf{F}}	
\newcommand{\mbG}{\mathbf{G}}	
\newcommand{\mbH}{\mathbf{H}}	
\newcommand{\mbI}{\mathbf{I}}	
\newcommand{\mbJ}{\mathbf{J}}	
\newcommand{\mbK}{\mathbf{K}}	
\newcommand{\mbL}{\mathbf{L}}	
\newcommand{\mbM}{\mathbf{M}}	
\newcommand{\mbN}{\mathbf{N}}	
\newcommand{\mbO}{\mathbf{O}}	
\newcommand{\mbP}{\mathbf{P}}	
\newcommand{\mbQ}{\mathbf{Q}}	
\newcommand{\mbR}{\mathbf{R}}	
\newcommand{\mbS}{\mathbf{S}}	
\newcommand{\mbT}{\mathbf{T}}	
\newcommand{\mbU}{\mathbf{U}}	
\newcommand{\mbV}{\mathbf{V}}	
\newcommand{\mbW}{\mathbf{W}}	
\newcommand{\mbX}{\mathbf{X}}	
\newcommand{\mbY}{\mathbf{Y}}	
\newcommand{\mbZ}{\mathbf{Z}}	
\newcommand{\R}{\mathds{R}}

\newcommand{\mbalpha}{\mathbold{\alpha}}	
\newcommand{\mbbeta}{\mathbold{\beta}}	
\newcommand{\mbdelta}{\mathbold{\delta}}	

\newcommand{\mbepsilon}{\mathbold{\epsilon}}	
\newcommand{\mbchi}{\mathbold{\chi}}	
\newcommand{\mbeta}{\mathbold{\eta}}	
\newcommand{\mbgamma}{\mathbold{\gamma}}	
\newcommand{\mbiota}{\mathbold{\iota}}	
\newcommand{\mbkappa}{\mathbold{\kappa}}	
\newcommand{\mblambda}{\mathbold{\lambda}}	
\newcommand{\mbmu}{\mathbold{\mu}}	
\newcommand{\mbnu}{\mathbold{\nu}}	
\newcommand{\mbomega}{\mathbold{\omega}}	
\newcommand{\mbphi}{\mathbold{\phi}}	
\newcommand{\mbpi}{\mathbold{\pi}}	
\newcommand{\mbpsi}{\mathbold{\psi}}	
\newcommand{\mbrho}{\mathbold{\rho}}	
\newcommand{\mbsigma}{\mathbold{\sigma}}	
\newcommand{\mbtau}{\mathbold{\tau}}	
\newcommand{\mbtheta}{\mathbold{\theta}}	
\newcommand{\mbupsilon}{\mathbold{\upsilon}}	
\newcommand{\mbvarepsilon}{\mathbold{\varepsilon}}	
\newcommand{\mbvarphi}{\mathbold{\varphi}}	
\newcommand{\mbvartheta}{\mathbold{\vartheta}}	
\newcommand{\mbvarrho}{\mathbold{\varrho}}	
\newcommand{\mbxi}{\mathbold{\xi}}	
\newcommand{\mbzeta}{\mathbold{\zeta}}	

\newcommand{\mbDelta}{\mathbold{\Delta}}	
\newcommand{\mbGamma}{\mathbold{\Gamma}}	
\newcommand{\mbLambda}{\mathbold{\Lambda}}	
\newcommand{\mbOmega}{\mathbold{\Omega}}	
\newcommand{\mbPhi}{\mathbold{\Phi}}	
\newcommand{\mbPi}{\mathbold{\Pi}}	
\newcommand{\mbPsi}{\mathbold{\Psi}}	
\newcommand{\mbSigma}{\mathbold{\Sigma}}	
\newcommand{\mbTheta}{\mathbold{\Theta}}	
\newcommand{\mbUpsilon}{\mathbold{\Upsilon}}	
\newcommand{\mbXi}{\mathbold{\Xi}}	

\newcommand{\rmdo}{\mathrm{do}}	
\newcommand{\rmP}{\mathrm{P}}
	
\newcommand{\indep}{\perp \!\!\! \perp}

\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{exercise}{Exercise}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
% \newtheorem{warning}{Warning}
\newtheorem{claim}{Claim}
\newtheorem{note}[remark]{Note}
\newtheorem{fact}[remark]{Fact}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator\supp{supp}

==> preamble/minimalist_bib.tex <==
\usepackage[%	
minnames=1,maxnames=99,maxcitenames=2,	
style=alphabetic,
doi=false,	
url=false,	
natbib,	
backend=bibtex,	
sorting=nyt	
]{biblatex}%	


\DeclareFieldFormat{sentencecase}{\MakeSentenceCase*{#1}}	

\renewbibmacro*{title}{%	
  \ifthenelse{\iffieldundef{title}\AND\iffieldundef{subtitle}}	
    {}	
    {\ifthenelse{\ifentrytype{article}\OR\ifentrytype{inbook}%	
      \OR\ifentrytype{incollection}\OR\ifentrytype{inproceedings}%	
      \OR\ifentrytype{inreference}}	
      {\printtext[title]{%	
        \printfield[sentencecase]{title}%	
        \setunit{\subtitlepunct}%	
        \printfield[sentencecase]{subtitle}}}%	
      {\printtext[title]{%	
        \printfield[titlecase]{title}%	
        \setunit{\subtitlepunct}%	
        \printfield[titlecase]{subtitle}}}%	
     \newunit}%	
  \printfield{titleaddon}}	



\AtEveryBibitem{%	
\ifentrytype{article}{	
    \clearfield{url}%	
    \clearfield{urldate}%	
    \clearfield{eprint}	
    \clearfield{eid}	
}{}	
\ifentrytype{book}{	
    \clearfield{url}%	
    \clearfield{urldate}%	
}{}	
\ifentrytype{collection}{	
    \clearfield{url}%	
    \clearfield{urldate}%	
}{}	
\ifentrytype{incollection}{	
    \clearfield{url}%	
    \clearfield{urldate}%	
}{}	
}	

\AtEveryBibitem{	
    \clearfield{pages}	
    \clearfield{review}%	
    \clearfield{series}%%	
    \clearfield{volume}	
    \clearfield{month}	
    \clearfield{eprint}	
    \clearfield{isbn}	
    \clearfield{issn}	
    \clearlist{location}	
    \clearfield{series}	
    \clearlist{publisher}	
    \clearname{editor}	
}{}	


==> preamble/preamble.tex <==
% ===== math stuff

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amscd}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{wrapfig}

% ===== color

%\usepackage[usenames,dvipsnames]{xcolor}

% ===== editing

\usepackage{lineno}
\setlength\linenumbersep{5pt}
\renewcommand\linenumberfont{\normalfont
  \tiny
  \sffamily
  \color{SkyBlue}}

% ===== nice to dos

% ===== figures

\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}

% ===== algorithms

\usepackage[algoruled]{algorithm2e}
\setlength{\interspacetitleruled}{8pt}

% ===== lists

\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    keywordstyle=\color{BurntOrange},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{darkblue},
    basicstyle=\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}

\usepackage{enumitem}
\renewcommand{\labelitemi}{{\color{black!30}\textbullet}}

% bibliography

% \usepackage{natbib}
\usepackage{hyperref}
\usepackage[all]{hypcap}
\hypersetup{colorlinks,linktoc=all}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}
\hypersetup{linkcolor=black}


% clever reference

\usepackage[nameinlink, capitalize]{cleveref}
\creflabelformat{equation}{#1#2#3}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\Crefname{appendix}{App.}{Apps.}
% \Crefname{section}{\S}{\S} %% KV: :) 
% acronyms and glossaries

\usepackage
[acronym,smallcaps,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper{}
\setglossarystyle{long3col}
\setlength\glsdescwidth{0.8\linewidth}
\setlength\glspagelistwidth{0pt}
\makeglossaries

% ===== useful packages

\usepackage{blindtext}
\usepackage{framed}

% ===== tables

\usepackage{booktabs}
\usepackage{multirow}
\usepackage{longtable}
\usepackage{etoolbox,siunitx}
\robustify\bfseries
\sisetup{detect-weight=true, detect-shape=true, detect-mode=true,
table-format=5.1, table-number-alignment=center}

% ===== other useful commands

\newcommand{\pp}{\noindent \textcolor{lightgray}{\P} \quad}

\newcommand{\draftdisclaimer}
{
  \begin{center}
    \begin{framed}
      DRAFT: DO NOT CITE OR DISTRIBUTE
    \end{framed}
  \end{center}
}

\newcommand{\important}[1]
{
  \vspace{0.1in}
  \begin{shaded}
    \textbf{#1}
  \end{shaded}
}

\newcommand{\q}[1]
{
  \red{{\sf Q | #1}}
}

\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}

% title

\newcommand{\mytitle}[2]{
  \begin{center}
    \large \textbf{#1} \\
    \normalsize
    \vspace{0.1in}
    #2 \\
    \vspace{0.25in}
    \today
    \vspace{0.25in}
  \end{center}
}



%
% %appendix
% \usepackage{appendix}
% \Crefname{appsec}{appendix}{appendices}
% \AtBeginEnvironment{appendices}{\crefalias{section}{appendix}}


